HST/FGS Trigonometric Parallaxes of M-dwarf Eclipsing Binaries

Hubble Space Telescope (HST) Fine Guidance Sensor (FGS) trigonometric parallax observations were obtained to directly determine distances to five nearby M-dwarf / M-dwarf eclipsing binary systems. These systems are intrinsically interesting as benchmark systems for establishing basic physical parameters for low-mass stars, such as luminosity L, and radius R. HST/FGS distances are also one of the few direct checks on Gaia trigonometric parallaxes, given the comparable sensitivity in both magnitude limit and determination of parallactic angles. A spectral energy distribution (SED) fit of each system's blended flux output was carried out, allowing for estimation of the bolometric flux from the primary and secondary components of each system. From the stellar M, L, and R values, the low-mass star relationships between L and M, and R and M, are compared against idealized expectations for such stars. An examination on the inclusion of these close M-dwarf/M-dwarf pairs in higher-order common proper motion (CPM) pairs is analysed; each of the 5 systems has indications of being part of a CPM system. Unexpected distances on interesting objects found within the grid of parallactic reference stars are also presented, including a nearby M dwarf and a white dwarf.

==> tables/astmodel_4par_ppmxl.tex <==
 \begin{deluxetable*}{lrcrcrcrc}
%\rotate
%\tabletypesize{\tiny}
\tabletypesize{\scriptsize}
\tablecaption{Final values after running gaussfit astrometric model using PPMXL proper motions as the initial estimates.}
\tablewidth{0pt}
\tablehead{
\colhead{Star} & \colhead{$\pi$} & \colhead{$\sigma_\pi$} & \colhead{$\mu_x$}  & \colhead{$\sigma_{\mu x}$} & \colhead{$\mu_y$}  & \colhead{$\sigma_{\mu y}$} & \colhead{$B-V$} & \colhead{$\sigma_{(B-V)}$} \\ 
\colhead{}     & \colhead{(mas)} & \colhead{(mas)}       & \colhead{(mas/yr)} & \colhead{(mas/yr)}       & \colhead{(mas/yr)} & \colhead{(mas/yr)}       & \colhead{(mag)} & \colhead{(mag)} }
\startdata
 ~2 (2)~~~YY-GEM          &   66.94  &   0.47 &  -211.190 &   0.67 &    -95.066 &   0.60 &   1.200 &   0.15  \\
 ~7 (7)~~~YY-GEM-REF1     &    0.79  &   0.06 &    -7.927 &   0.61 &     -0.960 &   0.54 &   1.095 &   0.01  \\
 ~8 (8)~~~YY-GEM-REF2     &    2.00  &   0.11 &    -5.811 &   1.14 &     -0.933 &   0.95 &   0.650 &   0.01  \\
 ~9 (9)~~~YY-GEM-REF3     &    1.17  &   0.04 &    -7.011 &   0.37 &      0.386 &   0.37 &   0.890 &   0.02  \\
 10 (10) YY-GEM-REF4      &    1.08  &   0.06 &    -6.102 &   0.83 &     -0.631 &   0.72 &   0.567 &   0.06  \\
 11 (11) YY-GEM-REF5      &          &        &           &        &            &        &         &         \\
 12 (12) YY-GEM-REF6      &          &        &           &        &            &        &         &         \\
 13 (13) YY-GEM-REF7      &    2.26  &   0.39 &   -12.484 &   1.19 &    -24.292 &   1.12 &   0.749 &   0.05  \\
\hline                                                                                                              
 ~5 (5)~~~NSVS0103        &   14.94  &   0.57 &  -107.340 &   2.01 &     58.454 &   1.98 &   1.499 &   0.12  \\
 33 (33) NSVS0103-REF00   &    2.08  &   0.15 &     2.376 &   3.79 &     16.675 &   3.86 &   0.771 &   0.01  \\
 34 (34) NSVS0103-REF01   &    1.52  &   0.08 &     3.300 &   1.49 &    -16.347 &   1.38 &   0.698 &   0.01  \\
 35 (35) NSVS0103-REF02   &    6.27  &   0.64 &   -38.111 &   1.35 &      8.773 &   1.58 &   0.692 &   0.01  \\
 36 (36) NSVS0103-REF05   &    2.12  &   0.09 &   -13.469 &   1.42 &     -2.261 &   1.63 &   0.917 &   0.01  \\
 37 (37) NSVS0103-REF19   &    1.33  &   0.29 &     6.340 &   3.23 &    -11.691 &   3.01 &   0.711 &   0.02  \\
 41 (41) NSVS0103-REF23   &    2.19  &   0.08 &     1.000 &   0.70 &     -4.100 &   0.70 &   0.573 &   0.01  \\
 39 (39) NSVS0103-REF68   &   14.88  &   0.70 &  -111.096 &   2.06 &     61.020 &   2.06 &   1.522 &   0.02  \\
 40 (40) NSVS0103-REF96   &    1.35  &   0.12 &    -6.846 &   1.19 &      2.960 &   1.08 &   0.502 &   0.01  \\
 \hline                                                                                                             
 ~1 (1)~~~GU-BOO          &    3.20  &   0.61 &    21.153 &   1.59 &    -27.529 &   1.54 &   1.252 &   0.01  \\
 20 (20) GU-BOO-REF01     &    2.09  &   0.12 &    -5.774 &   1.62 &      0.672 &   1.49 &   0.914 &   0.01  \\
 21 (21) GU-BOO-REF05     &    1.57  &   0.08 &   -14.763 &   1.79 &     12.578 &   1.57 &   0.948 &   0.02  \\
 22 (22) GU-BOO-REF08     &    1.44  &   0.24 &  -104.010 &   2.97 &      3.105 &   2.24 &   0.590 &   0.02  \\
 19 (19) GU-BOO-REF25     &    2.07  &   0.12 &    -2.832 &   1.64 &     -2.258 &   1.61 &   1.019 &   0.02  \\
 18 (18) GU-BOO-REF51     &    4.93  &   0.21 &   -11.191 &   2.00 &     18.999 &   1.49 &   1.035 &   0.01  \\
 15 (15) GU-BOO-REF53     &    0.92  &   0.03 &     3.593 &   1.12 &    -16.174 &   1.18 &   0.569 &   0.01  \\
 14 (14) GU-BOO-REF57     &    0.68  &   0.05 &    -3.323 &   1.52 &     -1.632 &   1.42 &   0.634 &   0.02  \\
\hline                                                                                                              
 53 (53) CM-DRA           &   68.42  &   0.44 & -1123.587 &   2.46 &   1182.487 &   2.99 &   1.532 &   0.00  \\
 55 (55) CM-DRA-REF45     &    2.49  &   0.24 &   -24.908 &   2.39 &      5.902 &   3.75 &   0.821 &   0.01  \\
 26 (26) CM-DRA-REF46     &    1.04  &   0.08 &   -10.103 &   2.49 &      3.958 &   4.34 &   0.618 &   0.01  \\
 54 (54) CM-DRA-REF47     &   66.41  &   1.62 & -1127.923 &   5.99 &   1201.907 &   4.37 &   0.473 &   0.03  \\
 29 (29) CM-DRA-REF58     &    1.38  &   0.09 &   -13.581 &   3.85 &    -16.638 &   4.17 &   0.700 &   0.01  \\
 30 (30) CM-DRA-REF65     &    1.30  &   0.10 &   -24.852 &   1.98 &    -13.061 &   3.18 &   0.849 &   0.02  \\
 31 (31) CM-DRA-REF66     &    1.74  &   0.21 &     3.516 &   3.33 &      3.243 &   3.36 &   0.554 &   0.02  \\
 32 (32) CM-DRA-REF94     &    0.15  &   0.01 &    -6.194 &   3.19 &      7.456 &   3.70 &   0.961 &   0.01  \\
\hline                                                                                                              
 ~6 (6)~~~TRES-HER0       &    5.78  &   0.55 &   -15.453 &   1.81 &     37.461 &   1.61 &   1.482 &   0.02  \\
 44 (44) TRES-HER0-REF337 &    2.17  &   0.16 &     2.719 &   0.76 &      7.848 &   0.66 &   0.467 &   0.01  \\
 46 (46) TRES-HER0-REF347 &    1.26  &   0.06 &     2.083 &   1.25 &      5.777 &   1.32 &   0.602 &   0.01  \\
 52 (52) TRES-HER0-REF363 &    2.99  &   0.10 &   -29.600 &   1.40 &     10.600 &   1.40 &   0.949 &   0.00  \\
 47 (47) TRES-HER0-REF377 &    2.68  &   0.19 &   -23.920 &   2.04 &     36.593 &   2.44 &   0.873 &   0.01  \\
 48 (48) TRES-HER0-REF380 &    0.44  &   0.03 &    -4.239 &   1.97 &    -13.743 &   2.21 &   0.557 &   0.01  \\
 49 (49) TRES-HER0-REF394 &    0.68  &   0.06 &    -3.367 &   1.31 &    -13.701 &   1.28 &   1.088 &   0.01  \\
 51 (51) TRES-HER0-REF823 &    0.44  &   0.52 &    -7.964 &   2.01 &    -12.535 &   2.21 &   0.748 &   0.05  \\
\enddata 
\label{tab.final_ppmxl}
\end{deluxetable*} 


==> tables/astmodel_4par_ucac4.tex <==
\begin{deluxetable*}{lrcrcrcrc}
%\rotate
%\tabletypesize{\tiny}
\tabletypesize{\scriptsize}
\tablecaption{Final values after running gaussfit astrometric model using UCAC4 proper motions as the initial estimates.}
\tablewidth{0pt}
\tablehead{
\colhead{Star} & \colhead{$\pi$} & \colhead{$\sigma_\pi$} & \colhead{$\mu_x$}  & \colhead{$\sigma_{\mu x}$} & \colhead{$\mu_y$}  & \colhead{$\sigma_{\mu y}$} & \colhead{$B-V$} & \colhead{$\sigma_{(B-V)}$} \\ 
\colhead{}     & \colhead{(mas)} & \colhead{(mas)}       & \colhead{(mas/yr)} & \colhead{(mas/yr)}       & \colhead{(mas/yr)} & \colhead{(mas/yr)}       & \colhead{(mag)} & \colhead{(mag)} }
\startdata
 ~2 (2)~~~YY-GEM          &   66.97  &   0.47 &  -206.594 &   0.60 &    -97.283 &   0.57 &   1.194 &   0.14  \\
 ~7 (7)~~~YY-GEM-REF1     &    0.79  &   0.06 &    -1.576 &   0.42 &     -2.927 &   0.34 &   1.095 &   0.01  \\
 ~8 (8)~~~YY-GEM-REF2     &    1.99  &   0.10 &    -1.266 &   0.95 &     -3.431 &   0.92 &   0.650 &   0.01  \\
 ~9 (9)~~~YY-GEM-REF3     &    1.17  &   0.05 &    -2.961 &   0.27 &     -2.272 &   0.28 &   0.890 &   0.03  \\
 10 (10) YY-GEM-REF4      &    1.08  &   0.05 &    -2.036 &   0.80 &     -3.218 &   0.68 &   0.570 &   0.05  \\
 11 (11) YY-GEM-REF5      &          &        &           &        &            &        &         &         \\
 12 (12) YY-GEM-REF6      &          &        &           &        &            &        &         &         \\
 13 (13) YY-GEM-REF7      &    1.81  &   0.62 &    -8.921 &   1.34 &    -25.387 &   1.12 &   0.765 &   0.09  \\
\hline                                                                                                              
 ~5 (5)~~~NSVS0103        &   15.10  &   0.58 &  -106.728 &   1.50 &     53.112 &   1.84 &   1.506 &   0.11  \\
 33 (33) NSVS0103-REF00   &    2.09  &   0.09 &     5.829 &   0.96 &      7.281 &   1.23 &   0.771 &   0.01  \\
 34 (34) NSVS0103-REF01   &    1.54  &   0.10 &     4.045 &   1.25 &    -19.460 &   1.40 &   0.698 &   0.01  \\
 35 (35) NSVS0103-REF02   &    6.44  &   0.63 &   -39.609 &   1.11 &      9.316 &   1.30 &   0.692 &   0.01  \\
 36 (36) NSVS0103-REF05   &    2.12  &   0.13 &    -9.775 &   1.63 &     -6.247 &   1.71 &   0.918 &   0.01  \\
 37 (37) NSVS0103-REF19   &    1.26  &   0.31 &     5.171 &   2.82 &    -10.686 &   2.75 &   0.713 &   0.03  \\
 41 (41) NSVS0103-REF23   &    2.19  &   0.08 &     3.800 &   0.67 &     -1.800 &   0.78 &   0.573 &   0.01  \\
 39 (39) NSVS0103-REF68   &   14.97  &   0.70 &  -110.570 &   1.82 &     56.855 &   1.99 &   1.522 &   0.02  \\
 40 (40) NSVS0103-REF96   &    1.34  &   0.12 &    -7.027 &   0.77 &      2.752 &   0.94 &   0.502 &   0.01  \\
\hline                                                                                                              
 ~1 (1)~~~GU-BOO          &    3.25  &   0.61 &    20.165 &   1.44 &    -24.669 &   1.50 &   1.252 &   0.01  \\
 20 (20) GU-BOO-REF01     &    2.08  &   0.13 &    -3.519 &   1.69 &      4.260 &   1.45 &   0.914 &   0.02  \\
 21 (21) GU-BOO-REF05     &    1.57  &   0.10 &   -16.428 &   1.58 &     16.426 &   2.04 &   0.949 &   0.03  \\
 22 (22) GU-BOO-REF08     &    1.39  &   0.20 &  -101.965 &   1.30 &      5.471 &   1.22 &   0.591 &   0.02  \\
 19 (19) GU-BOO-REF25     &    2.06  &   0.10 &    -2.316 &   1.41 &      0.594 &   1.53 &   1.019 &   0.01  \\
 18 (18) GU-BOO-REF51     &    4.93  &   0.19 &   -12.727 &   0.82 &     19.902 &   0.84 &   1.035 &   0.01  \\
 15 (15) GU-BOO-REF53     &    0.92  &   0.04 &     2.091 &   1.32 &    -12.980 &   1.21 &   0.570 &   0.01  \\
 14 (14) GU-BOO-REF57     &    0.68  &   0.06 &    -4.527 &   1.35 &      0.860 &   1.39 &   0.634 &   0.03  \\
\hline                                                                                                              
 53 (53) CM-DRA           &   68.39  &   0.45 & -1119.004 &   0.91 &   1182.574 &   0.88 &   1.532 &   0.00  \\
 55 (55) CM-DRA-REF45     &    2.51  &   0.23 &   -16.324 &   0.76 &     10.977 &   2.29 &   0.821 &   0.01  \\
 26 (26) CM-DRA-REF46     &    1.04  &   0.10 &    -3.740 &   1.49 &      5.667 &   2.75 &   0.618 &   0.01  \\
 54 (54) CM-DRA-REF47     &   65.05  &   2.63 & -1128.561 &   5.61 &   1192.031 &  10.00 &   0.472 &   0.03  \\
 29 (29) CM-DRA-REF58     &    1.37  &   0.10 &   -14.359 &   1.37 &     -1.013 &   1.74 &   0.700 &   0.02  \\
 30 (30) CM-DRA-REF65     &    1.30  &   0.09 &   -15.948 &   1.03 &     -8.566 &   1.09 &   0.849 &   0.02  \\
 31 (31) CM-DRA-REF66     &    1.55  &   0.15 &    -0.738 &   1.26 &     14.028 &   1.07 &   0.555 &   0.01  \\
 32 (32) CM-DRA-REF94     &    0.15  &   0.01 &    -1.617 &   0.88 &      2.803 &   0.74 &   0.960 &   0.01  \\
\hline                                                                                                              
 ~6 (6)~~~TRES-HER0       &    5.66  &   0.57 &   -16.010 &   1.80 &     34.026 &   1.23 &   1.482 &   0.02  \\
 44 (44) TRES-HER0-REF337 &    2.17  &   0.14 &     3.348 &   0.25 &      4.336 &   0.64 &   0.467 &   0.00  \\
 46 (46) TRES-HER0-REF347 &    1.30  &   0.11 &     1.068 &   1.30 &      4.003 &   1.32 &   0.602 &   0.01  \\
 52 (52) TRES-HER0-REF363 &    2.99  &   0.10 &   -36.300 &   0.78 &      5.100 &   2.33 &   0.949 &   0.00  \\
 47 (47) TRES-HER0-REF377 &    2.68  &   0.18 &   -27.581 &   1.86 &     33.751 &   1.33 &   0.873 &   0.01  \\
 48 (48) TRES-HER0-REF380 &    0.43  &   0.02 &    -7.014 &   1.67 &    -15.843 &   1.07 &   0.557 &   0.00  \\
 49 (49) TRES-HER0-REF394 &    0.68  &   0.05 &     0.685 &   0.93 &    -15.271 &   0.49 &   1.088 &   0.01  \\
 51 (51) TRES-HER0-REF823 &    0.43  &   0.53 &   -10.502 &   1.95 &    -14.482 &   1.54 &   0.746 &   0.05  \\
\enddata 
\label{tab.final_ucac4}
\end{deluxetable*} 


==> tables/ref_stars_distances-old.tex <==
%% LaTeX deluxetable generator for the AASTeX package.
%% Written by Greg Schwarz (5/1/2001).

%% Table generated: Mon Sep  6 22:47:06 2010

%% Remove the two lines and the last line if you want
%% want to incorporate this table into another LaTex document.

%\documentclass[twocolumn]{emulateapj}
%\begin{document}

%% The values (usually only l,r and c) in the last part of
%% \begin{deluxetable}{} command tell LaTeX how many columns
%% there are and how to align them.

%\clearpage
%\LongTables % optionally
%\begin{landscape}
%\begin{deluxetable}{lccccl}

\begin{deluxetable*}{lcccccccccc}

%% Keep a portrait orientation

%% Over-ride the default font size
%% Use Default (12pt)

%% Use \tablewidth{?pt} to over-ride the default table width.
%% If you are unhappy with the default look at the end of the
%% *.log file to see what the default was set at before adjusting
%% this value.

%% This is the title of the table.
\tablecaption{\label{tab_refStarsDist}Estimated distances for reference stars.}

%% This command over-rides LaTeX's natural table count
%% and replaces it with this number.  LaTeX will increment
%% all other tables after this table based on this number
%\tablenum{1}

%% The \tablehead gives provides the column headers.  It
%% is currently set up so that the column labels are on the
%% top line and the units surrounded by ()s are in the
%% bottom line.  You may add more header information by writing
%% another line between these lines. For each column that requries
%% extra information be sure to include a \colhead{text} command
%% and remember to end any extra lines with \\ and include the
%% correct number of &s. 
\tablehead{
\colhead{Program ID} & 
\colhead{Ang. Size} & 
\colhead{$F_{\rm BOL}$} &
\colhead{$A_V$} &
\colhead{Sp. Type} &
\colhead{$R$} &
\colhead{$d_{\rm R}$} &
\colhead{$M_V$} &
\colhead{$BC$} &
\colhead{$d_{\rm MV}$} &
\colhead{$d_{\rm final}$} \\
\colhead{} &
\colhead{(mas)} &
\colhead{} &
\colhead{(mag)} &
\colhead{} &
\colhead{$(R_\odot)$} &
\colhead{(pc)} &
\colhead{(mag)} &
\colhead{(mag)} &
\colhead{(pc)} &
\colhead{(pc)}
}

%% All data must appear between the \startdata and \enddata commands
\startdata
CM-DRA-REF45 & 0.0264 & 1.872E-10 & 0.42 & G8V? & 0.88 & 311 & 5.5 & -0.4 & 287 & 299 \\
CM-DRA-REF46 & 0.0128 & 5.493E-11 & 0.36 & G2V & 1.00 & 726 & 4.7 & -0.2 & 715 & 721 \\
CM-DRA-REF58 & 0.0130 & 5.481E-11 & 0.56 & G5-G6V & 0.93 & 667 & 5.1 & -0.2 & 546 & 606 \\
CM-DRA-REF65 & 0.0102 & 2.508E-11 & 0.00 & K0V & 0.85 & 775 & 5.9 & -0.3 & 758 & 767 \\
CM-DRA-REF66 & 0.0211 & 1.975E-10 & 0.12 & F9V & 1.08 & 474 & 4.2 & -0.2 & 524 & 499 \\
CM-DRA-REF94 & 0.0190 & 6.673E-11 & 0.00 & K0III & 15.00 & 7,336 & 0.7 & -0.5 & 5,560 & 6,448 \\
GU-BOO-REF01 & 0.0152 & 5.540E-11 & 0.25 & K0V & 0.85 & 520 & 5.9 & -0.3 & 455 & 487 \\
GU-BOO-REF05 & 0.0108 & 2.841E-11 & 0.23 & K0-K2V & 0.85 & 732 & 5.9 & -0.3 & 640 & 686 \\
GU-BOO-REF08 & 0.0168 & 1.259E-10 & 0.54 & F9V & 1.08 & 595 & 4.2 & -0.2 & 541 & 568 \\
GU-BOO-REF25 & 0.0163 & 3.606E-11 & 0.14 & K3V & 0.78 & 447 & 6.7 & -0.5 & 449 & 448 \\
GU-BOO-REF51 & 0.0374 & 1.910E-10 & 0.00 & K3V & 0.78 & 195 & 6.7 & -0.5 & 208 & 201 \\
GU-BOO-REF53 & 0.0106 & 4.296E-11 & 0.07 & G0V & 1.05 & 918 & 4.4 & -0.2 & 1,052 & 985 \\
GU-BOO-REF57 & 0.0078 & 2.031E-11 & 0.00 & G2V & 1.00 & 1,196 & 4.7 & -0.2 & 1,391 & 1,294 \\
NSVS0103-REF00 & 0.0186 & 9.300E-11 & 0.00 & G8V & 0.88 & 441 & 5.5 & -0.4 & 493 & 467 \\
NSVS0103-REF01 & 0.0134 & 5.809E-11 & 0.00 & G5V & 0.93 & 647 & 5.1 & -0.2 & 687 & 667 \\
NSVS0103-REF02 & 0.0698 & 1.578E-09 & 0.26 & G5V & 0.93 & 124 & 5.1 & -0.2 & 117 & 121 \\
NSVS0103-REF05 & 0.0148 & 4.183E-11 & 0.00 & K2V & 0.81 & 506 & 6.4 & -0.4 & 490 & 498 \\
NSVS0103-REF19 & 0.0186 & 1.159E-10 & 0.06 & G3V & 0.98 & 488 & 4.8 & -0.2 & 533 & 510 \\
NSVS0103-REF23 & 0.0263 & 2.611E-10 & 0.19 & G0V & 1.05 & 370 & 4.4 & -0.2 & 405 & 388 \\
NSVS0103-REF68 & 0.0558 & 9.742E-11 & 0.00 & M4.5V & 0.37 & 62 & 11.5 & -2.5 & 78 & 70 \\
NSVS0103-REF96 & 0.0186 & 1.799E-10 & 0.00 & F6V & 1.17 & 584 & 3.7 & -0.1 & 734 & 659 \\
TRES-HER0-REF337 & 0.0365 & 8.097E-10 & 0.07 & F5V & 1.20 & 306 & 3.5 & -0.1 & 361 & 333 \\
TRES-HER0-REF347 & 0.0158 & 9.490E-11 & 0.11 & G0V & 1.05 & 616 & 4.4 & -0.2 & 697 & 656 \\
TRES-HER0-REF363 & 0.0235 & 7.551E-11 & 0.00 & K3V & 0.78 & 310 & 6.7 & -0.5 & 330 & 320 \\
TRES-HER0-REF377 & 0.0225 & 1.217E-10 & 0.00 & K0V & 0.85 & 352 & 5.9 & -0.3 & 344 & 348 \\
TRES-HER0-REF380 & 0.0109 & 7.231E-11 & 0.06 & F8III & 5.09 & 4,341 & 0.0 & 0.0 & 5,702 & 5,021 \\
TRES-HER0-REF394 & 0.1050 & 1.457E-09 & 0.00 & K2IIIab & 18.40 & 1,628 & 0.5 & -0.6 & 1,372 & 1,500 \\
TRES-HER0-REF823 & 0.0109 & 3.984E-11 & 2.36 & G2V & 1.00 & 852 & 4.7 & -0.2 & 336 & 594 \\
YY-GEM-REF1 & 0.0878 & 1.424E-09 & 0.42 & K0IIIb & 15.00 & 1,587 & 0.7 & -0.5 & 993 & 1,290 \\
YY-GEM-REF2 & 0.0219 & 1.611E-10 & 0.00 & G3V & 0.98 & 415 & 4.8 & -0.2 & 465 & 440 \\
YY-GEM-REF3 & 0.1360 & 3.421E-09 & 0.04 & K0III & 15.00 & 1,025 & 0.7 & -0.5 & 763 & 894 \\
YY-GEM-REF4 & 0.0118 & 5.288E-11 & 0.00 & G0V & 1.05 & 825 & 4.4 & -0.2 & 981 & 903 \\
YY-GEM-REF5 & 0.0047 & 8.484E-12 & 0.00 & G0V & 1.05 & 2,057 & 4.4 & -0.2 & 2,449 & 2,253 \\

\enddata

%% Include any \tablenotetext{key}{text}, \tablerefs{ref list},
%% or \tablecomments{text} between the \enddata and
%% \end{deluxetable} commands

%% No \tablecomments indicated

%% No \tablerefs indicated

\end{deluxetable*}

%\end{document}

%\end{deluxetable}
%\clearpage
%\end{landscape}


==> tables/ref_stars_information.old.tex <==
%% LaTeX deluxetable generator for the AASTeX package.
%% Written by Greg Schwarz (5/1/2001).

%% Table generated: Mon Sep  6 22:47:06 2010

%% Remove the two lines and the last line if you want
%% want to incorporate this table into another LaTex document.

%\documentclass[twocolumn]{emulateapj}
%\begin{document}

%% The values (usually only l,r and c) in the last part of
%% \begin{deluxetable}{} command tell LaTeX how many columns
%% there are and how to align them.

\clearpage
\LongTables % optionally
\begin{landscape}
%\begin{deluxetable}{lccccl}

\begin{deluxetable*}{lccccccccccl}

%% Keep a portrait orientation

%% Over-ride the default font size
%% Use Default (12pt)

%% Use \tablewidth{?pt} to over-ride the default table width.
%% If you are unhappy with the default look at the end of the
%% *.log file to see what the default was set at before adjusting
%% this value.

%% This is the title of the table.
\tablecaption{\label{tab_photometry}Observed targets, coordinates, number of visibility points, and resultant uniform disk angular size.}

%% This command over-rides LaTeX's natural table count
%% and replaces it with this number.  LaTeX will increment
%% all other tables after this table based on this number
%\tablenum{1}

%% The \tablehead gives provides the column headers.  It
%% is currently set up so that the column labels are on the
%% top line and the units surrounded by ()s are in the
%% bottom line.  You may add more header information by writing
%% another line between these lines. For each column that requries
%% extra information be sure to include a \colhead{text} command
%% and remember to end any extra lines with \\ and include the
%% correct number of &s.
\tablehead{\colhead{Program ID} & \colhead{RA} & \colhead{DE}
& \colhead{U}& \colhead{B}& \colhead{V}& \colhead{R}
& \colhead{I} & \colhead{J} & \colhead{H} & \colhead{K} & \colhead{Spectral}\\
\colhead{} & \colhead{(hms)} & \colhead{(dms)} & \colhead{(mag)} & \colhead{(mag)} & \colhead{(mag)} & \colhead{(mag)} & \colhead{(mag)} & \colhead{(mag)} & \colhead{(mag)} & \colhead{(mag)} & \colhead{Type} }

%% All data must appear between the \startdata and \enddata commands
\startdata
CM-DRA & 16 34 20.417 & +57 09 43.93 & \ldots & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 7.80 & M4.5V \\
CM-DRA-REF45 & 16 33 57.786 & +57 14 23.13 & 0.00 & 0.00 & 13.51 & 0.00 & 0.00 & 0.00 & 0.00 & 11.21 & G8V?  \\
CM-DRA-REF46 & 16 33 55.605 & +57 14 23.16 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 12.75 & G2V  \\
CM-DRA-REF47 & 16 34 22.591 & +57 09 59.81 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & wd \\
CM-DRA-REF58 & 16 33 44.447 & +57 12 46.29 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 12.75 & G5-G6V  \\
CM-DRA-REF65 & 16 34 22.925 & +57 11 46.70 & 0.00 & 0.00 & 15.17 & 0.00 & 0.00 & 0.00 & 0.00 & 13.33 & K0V  \\
CM-DRA-REF66 & 16 33 48.569 & +57 11 40.86 & 0.00 & 0.00 & 13.01 & 0.00 & 0.00 & 0.00 & 0.00 & 11.53 & F9V  \\
CM-DRA-REF94 & 16 34 24.625 & +57 08 26.94 & 0.00 & 0.00 & 14.26 & 0.00 & 0.00 & 0.00 & 0.00 & 11.94 & K0III  \\
GU-BOO & 15 21 54.838 & +33 56 09.25 & 0.00 & 0.00 & 13.60 & 0.00 & 0.00 & 0.00 & 0.00 & 10.22 & M0/M1.5V \\
GU-BOO-REF01 & 15 22 01.145 & +34 01 05.89 & 0.00 & 0.00 & 14.54 & 0.00 & 0.00 & 0.00 & 0.00 & 12.44 & K0V  \\
GU-BOO-REF05 & 15 21 50.732 & +34 00 32.70 & 0.00 & 0.00 & 15.25 & 0.00 & 0.00 & 0.00 & 0.00 & 13.13 & K0-K2V  \\
GU-BOO-REF08 & 15 22 05.555 & +34 00 02.18 & 0.00 & 0.00 & 13.74 & 0.00 & 0.00 & 0.00 & 0.00 & 12.03 & F9V  \\
GU-BOO-REF25 & 15 21 58.531 & +34 00 10.86 & 0.00 & 0.00 & 15.14 & 0.00 & 0.00 & 0.00 & 0.00 & 12.57 & K3V  \\
GU-BOO-REF51 & 15 22 20.585 & +33 52 14.83 & 0.00 & 0.00 & 13.34 & 0.00 & 0.00 & 0.00 & 0.00 & 10.77 & K3V  \\
GU-BOO-REF53 & 15 21 56.870 & +33 58 37.57 & 0.00 & 0.00 & 14.44 & 0.00 & 0.00 & 0.00 & 0.00 & 13.08 & G0V  \\
GU-BOO-REF57 & 15 21 57.397 & +33 55 29.10 & 0.00 & 0.00 & 15.05 & 0.00 & 0.00 & 0.00 & 0.00 & 13.77 & G2V  \\
NSVS0103 & 13 45 34.953 & +79 23 48.61 & 0.00 & 0.00 & 13.38 & 0.00 & 0.00 & 0.00 & 0.00 & 8.78 & M2-M3V \\
NSVS0103-REF00 & 13 44 02.121 & +79 23 49.48 & 0.00 & 0.00 & 13.47 & 0.00 & 0.00 & 0.00 & 0.00 & 11.96 & G8V  \\
NSVS0103-REF01 & 13 46 21.316 & +79 21 34.95 & 0.00 & 0.00 & 13.84 & 0.00 & 0.00 & 0.00 & 0.00 & 12.59 & G5V  \\
NSVS0103-REF02 & 13 47 30.350 & +79 23 37.52 & 0.00 & 0.00 & 10.78 & 0.00 & 0.00 & 0.00 & 0.00 & 9.05 & G5V  \\
NSVS0103-REF05 & 13 45 41.357 & +79 21 05.38 & 0.00 & 0.00 & 14.16 & 0.00 & 0.00 & 0.00 & 0.00 & 12.49 & K2V  \\
NSVS0103-REF19 & 13 46 37.263 & +79 18 47.62 & 0.00 & 0.00 & 13.37 & 0.00 & 0.00 & 0.00 & 0.00 & 11.79 & G3V  \\
NSVS0103-REF23 & 13 45 20.334 & +79 18 01.73 & 0.00 & 0.00 & 12.80 & 0.00 & 0.00 & 0.00 & 0.00 & 11.17 & G0V  \\
NSVS0103-REF68 & 13 45 55.139 & +79 23 14.00 & 0.00 & 0.00 & 15.30 & 0.00 & 0.00 & 0.00 & 0.00 & 10.76 & M4.5V  \\
NSVS0103-REF96 & 13 46 58.399 & +79 22 04.23 & 0.00 & 0.00 & 12.77 & 0.00 & 0.00 & 0.00 & 0.00 & 11.70 & F6V  \\
TRES-HER0 & 16 50 20.771 & +46 39 01.61 & 0.00 & 0.00 & 15.47 & 0.00 & 0.00 & 0.00 & 0.00 & 10.88 & M2-M3 V \\
TRES-HER0-REF337 & 16 50 03.823 & +46 43 17.02 & 0.00 & 0.00 & 11.36 & 0.00 & 0.00 & 0.00 & 0.00 & 10.16 & F5V  \\
TRES-HER0-REF347 & 16 50 13.877 & +46 41 26.68 & 0.00 & 0.00 & 13.71 & 0.00 & 0.00 & 0.00 & 0.00 & 12.26 & G0V  \\
TRES-HER0-REF363 & 16 50 58.817 & +46 38 49.20 & 0.00 & 0.00 & 13.96 & 0.00 & 0.00 & 0.00 & 0.00 & 11.77 & K3V  \\
TRES-HER0-REF377 & 16 50 50.869 & +46 36 46.17 & 0.00 & 0.00 & 13.57 & 0.00 & 0.00 & 0.00 & 0.00 & 11.55 & K0V  \\
TRES-HER0-REF380 & 16 50 48.218 & +46 36 32.09 & 0.00 & 0.00 & 13.95 & 0.00 & 0.00 & 0.00 & 0.00 & 12.72 & F8III  \\
TRES-HER0-REF394 & 16 49 56.216 & +46 33 36.03 & 0.00 & 0.00 & 10.82 & 0.00 & 0.00 & 0.00 & 0.00 & 8.39 & K2IIIab  \\
TRES-HER0-REF823 & 16 50 44.114 & +46 37 11.08 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 13.44 & G2V  \\
YY-GEM & 07 34 37.446 & +31 52 10.22 & 0.00 & 0.00 & 10.72 & 0.00 & 0.00 & 0.00 & 0.00 & 5.24 & M1.0Ve \\
YY-GEM-REF1 & 07 34 52.068 & +31 52 34.14 & 0.00 & 0.00 & 11.64 & 0.00 & 0.00 & 0.00 & 0.00 & 8.69 & K0IIIb  \\
YY-GEM-REF2 & 07 34 49.027 & +31 51 42.87 & 0.00 & 0.00 & 12.96 & 0.00 & 0.00 & 0.00 & 0.00 & 11.49 & G3V  \\
YY-GEM-REF3 & 07 34 26.315 & +31 51 00.12 & 0.00 & 0.00 & 9.96 & 0.00 & 0.00 & 0.00 & 0.00 & 7.69 & K0III  \\
YY-GEM-REF4 & 07 34 31.213 & +31 51 16.65 & 0.00 & 0.00 & 14.00 & 0.00 & 0.00 & 0.00 & 0.00 & 12.89 & G0V  \\
YY-GEM-REF5 & 07 34 41.849 & +31 51 37.15 & 0.00 & 0.00 & 12.64 & 0.00 & 0.00 & 0.00 & 0.00 & 14.78 & G0V  \\
YY-GEM-REF6 & 07 34 42.028 & +31 51 58.49 & 0.00 & 0.00 & 13.02 & 0.00 & 0.00 & 0.00 & 0.00 & 14.37 & G2V  \\
YY-GEM-REF7 & 07 34 31.228 & +31 52 29.27 & 0.00 & 0.00 & 9.89 & 0.00 & 0.00 & 0.00 & 0.00 & 11.89 & G8V  \\
\enddata

%% Include any \tablenotetext{key}{text}, \tablerefs{ref list},
%% or \tablecomments{text} between the \enddata and
%% \end{deluxetable} commands

%% No \tablecomments indicated

%% No \tablerefs indicated

\end{deluxetable*}

%\end{document}

%\end{deluxetable}
\clearpage
\end{landscape}


==> tables/refstar_coord_pm_par.tex <==
\begin{deluxetable*}{lccccccccc}
%\rotate
\tabletypesize{\tiny}
%\tabletypesize{\scriptsize}
\tablecaption{Initial star data used as constraints in the gaussfit astrometric model.}
\tablewidth{0pt}
\tablehead{
\colhead{Star} & \colhead{RA}      & \colhead{DEC}     & \colhead{pmRA}     & \colhead{pmDEC}    & \colhead{pmRA}     & \colhead{pmDEC}    & \colhead{pmRA}     & \colhead{pmDEC}    & \colhead{$\pi_{\rm est}$} \\
\colhead{}     & \colhead{URAT1}   & \colhead{URAT1}   & \colhead{URAT1}    & \colhead{URAT1}    & \colhead{UCAC4}    & \colhead{UCAC4}    & \colhead{PPMXL}    & \colhead{PPMXL}    & \colhead{(mas)}         \\
\colhead{}     & \colhead{(J2000)} & \colhead{(J2000)} & \colhead{(mas/yr)} & \colhead{(mas/yr)} & \colhead{(mas/yr)} & \colhead{(mas/yr)} & \colhead{(mas/yr)} & \colhead{(mas/yr)} & \colhead{}    }                
\startdata
(2)  YY-GEM       &  07 34 37.616 & +31 52 11.30 &  -197.3 $\pm$ 5.5 & -90.7 $\pm$ 5.5 & -202.9  $\pm$  1.5 &   -97.0  $\pm$  1.6 &    -200.2 $\pm$  1.2  &   -92.5 $\pm$  1.3  &                       \\
(7)  YY-GEM-REF1  &  07 34 52.061 & +31 52 34.13 &  ~~~9.5 $\pm$ 5.4 & ~-1.1 $\pm$ 5.4 & ~~-1.5  $\pm$  1.3 &   ~-2.9  $\pm$  1.1 &    ~~-8.1 $\pm$  1.7  &   ~-0.9 $\pm$  1.7  &   0.804 $\pm$  0.187  \\
(8)  YY-GEM-REF2  &  07 34 49.016 & +31 51 42.85 &  ~~11.5 $\pm$ 5.4 & ~-2.6 $\pm$ 5.4 & ~~-2.4  $\pm$  3.0 &   ~-4.7  $\pm$  3.4 &    ~~-3.6 $\pm$  3.4  &   ~-2.0 $\pm$  3.4  &   1.952 $\pm$  0.195  \\
(9)  YY-GEM-REF3  &  07 34 26.314 & +31 51 00.16 &  ~~-1.0 $\pm$ 5.4 & ~-7.3 $\pm$ 5.4 & ~~-2.9  $\pm$  0.8 &   ~-2.3  $\pm$  0.9 &    ~~-7.0 $\pm$  1.3  &   ~~0.4 $\pm$  1.3  &   1.171 $\pm$  0.145  \\
(10) YY-GEM-REF4  &  07 34 31.215 & +31 51 16.67 &  ~~~6.7 $\pm$ 5.4 & ~-6.3 $\pm$ 5.4 & ~~-5.5  $\pm$  6.4 &   ~-4.1  $\pm$  5.5 &    ~-15.3 $\pm$ 13.6  &   ~~8.5 $\pm$ 13.6  &   1.074 $\pm$  0.107  \\
(11) YY-GEM-REF5  &  07 34 41.840 & +31 51 37.18 &  ~~~4.4 $\pm$ 5.5 & ~-6.3 $\pm$ 5.5 &                    &                     &                       &                     &   0.441 $\pm$  0.048  \\
(12) YY-GEM-REF6  &  07 34 42.026 & +31 51 58.52 &  ~~21.4 $\pm$ 5.4 & -12.1 $\pm$ 5.4 &                    &                     &                       &                     &   0.552 $\pm$  0.055  \\
(13) YY-GEM-REF7  &  07 34 31.234 & +31 52 29.36 &  ~~~6.1 $\pm$ 5.4 & -27.9 $\pm$ 5.4 & ~-21.0  $\pm$  5.6 &   -21.6  $\pm$  2.5 &    ~-19.1 $\pm$ 19.6  &   -37.2 $\pm$ 19.6  &   2.536 $\pm$  0.677  \\
\hline                                                                                                          
(5)\phantom{3} NSVS0103 &  13 45 34.863 & +79 23 48.32  &  -106.3 $\pm$ 5.6 & ~58.0 $\pm$ 5.6 & -105.5  $\pm$  5.6 &   ~57.3  $\pm$  2.7 &    -107.2 $\pm$  4.6  &   ~62.3 $\pm$  4.6  &                       \\
(33) NSVS0103-REF00     &  13 44 02.078 & +79 23 49.25  &  ~~10.0 $\pm$ 5.6 & ~~9.2 $\pm$ 5.6 & ~~~5.6  $\pm$  2.1 &   ~~6.9  $\pm$  2.6 &    ~~-3.3 $\pm$  5.5  &   ~11.0 $\pm$  5.5  &   2.089 $\pm$  0.209  \\
(34) NSVS0103-REF01     &  13 46 21.283 & +79 21 34.78  &  ~~~5.7 $\pm$ 5.6 & -17.5 $\pm$ 5.6 & ~~~3.1  $\pm$  2.4 &   -21.2  $\pm$  3.1 &    ~~~2.3 $\pm$  4.0  &   -15.5 $\pm$  4.0  &   1.492 $\pm$  0.149  \\
(35) NSVS0103-REF02     &  13 47 30.341 & +79 23 37.52  &  ~-39.0 $\pm$ 5.6 & ~12.1 $\pm$ 5.6 & ~-39.1  $\pm$  1.5 &   ~~7.9  $\pm$  1.7 &    ~-37.8 $\pm$  1.8  &   ~~6.7 $\pm$  1.8  &   7.593 $\pm$  0.759  \\
(36) NSVS0103-REF05     &  13 45 41.324 & +79 21 05.32  &  ~~-5.9 $\pm$ 5.5 & ~-8.6 $\pm$ 5.5 & ~~-8.0  $\pm$  3.7 &   ~-8.6  $\pm$  3.8 &    ~-13.4 $\pm$  4.0  &   ~-2.9 $\pm$  4.0  &   2.129 $\pm$  0.213  \\
(37) NSVS0103-REF19     &  13 46 37.229 & +79 18 47.58  &  ~~-6.1 $\pm$ 5.6 & ~-0.2 $\pm$ 5.6 & ~~-3.5  $\pm$  2.3 &   ~-0.4  $\pm$  3.0 &    ~~-6.6 $\pm$  4.0  &   ~~4.3 $\pm$  4.0  &   1.759 $\pm$  0.226  \\
(41) NSVS0103-REF23     &  13 45 19.615 & +79 18 02.02  &  ~~10.9 $\pm$ 5.5 & ~~3.3 $\pm$ 5.5 & ~~~3.8  $\pm$  1.8 &   ~-1.8  $\pm$  2.1 &    ~~~1.0 $\pm$  1.9  &   ~-4.1 $\pm$  1.9  &   2.193 $\pm$  0.219  \\
(39) NSVS0103-REF68     &  13 45 55.082 & +79 23 13.83  &  -107.1 $\pm$ 5.6 & ~61.7 $\pm$ 5.6 & ~-31.1  $\pm$  4.7 &   ~13.1  $\pm$  5.4 &    -111.6 $\pm$  4.0  &   ~60.2 $\pm$  4.0  &  18.315 $\pm$ 10.868  \\
(40) NSVS0103-REF96     &  13 46 58.297 & +79 22 04.30  &  ~~-7.3 $\pm$ 5.5 & ~~3.7 $\pm$ 5.5 & ~~-6.5  $\pm$  1.2 &   ~~3.6  $\pm$  1.3 &    ~~-5.6 $\pm$  1.9  &   ~~3.8 $\pm$  1.9  &   1.297 $\pm$  0.187  \\
\hline                                                                                                                                 
(1)\phantom{2} GU-BOO   &  15 21 54.828&  +33 56 08.85  &  ~~17.4 $\pm$ 5.9 & -12.3 $\pm$ 5.9 & ~~21.1  $\pm$  2.0 &   -28.3  $\pm$  2.4 &    ~~20.1 $\pm$  3.6  &   -33.6 $\pm$  3.6  &                       \\
(20) GU-BOO-REF01       &  15 22 01.147&  +34 01 05.74  &  ~-12.3 $\pm$ 5.9 & ~~8.1 $\pm$ 5.9 & ~~-0.3  $\pm$  3.9 &   ~~5.2  $\pm$  3.0 &    ~~-8.4 $\pm$  3.6  &   ~~0.2 $\pm$  3.6  &   2.138 $\pm$  0.214  \\
(21) GU-BOO-REF05       &  15 21 50.742&  +34 00 32.57  &  ~-25.9 $\pm$ 5.9 & ~25.1 $\pm$ 5.9 & ~-17.6  $\pm$  3.4 &   ~12.6  $\pm$  4.0 &    ~-13.3 $\pm$  3.6  &   ~11.7 $\pm$  3.6  &   1.581 $\pm$  0.158  \\
(22) GU-BOO-REF08       &  15 22 05.546&  +34 00 01.69  &  -105.6 $\pm$ 5.9 & ~16.1 $\pm$ 5.9 & -101.2  $\pm$  2.2 &   ~~5.8  $\pm$  2.5 &    -101.0 $\pm$  3.6  &   ~~4.3 $\pm$  3.6  &   1.275 $\pm$  0.341  \\
(19) GU-BOO-REF25       &  15 21 58.537&  +34 00 10.68  &  ~-10.8 $\pm$ 5.8 & ~11.1 $\pm$ 5.8 & ~~-3.4  $\pm$  3.5 &   ~~2.0  $\pm$  4.0 &    ~~-5.3 $\pm$  3.6  &   ~~0.1 $\pm$  3.6  &   2.037 $\pm$  0.204  \\
(18) GU-BOO-REF51       &  15 22 20.588&  +33 52 14.81  &  ~-15.3 $\pm$ 5.2 & ~18.1 $\pm$ 5.2 & ~-13.0  $\pm$  1.9 &   ~20.1  $\pm$  2.1 &    ~-12.3 $\pm$  3.7  &   ~18.9 $\pm$  3.7  &   4.950 $\pm$  0.495  \\
(15) GU-BOO-REF53       &  15 21 56.880&  +33 58 37.45  &  ~~-2.0 $\pm$ 5.9 & ~-5.6 $\pm$ 5.9 & ~~~1.1  $\pm$  2.9 &   -12.8  $\pm$  3.6 &    ~~~3.6 $\pm$  3.6  &   -15.6 $\pm$  3.6  &   0.916 $\pm$  0.092  \\
(14) GU-BOO-REF57       &  15 21 57.404&  +33 55 28.90  &  ~~-8.6 $\pm$ 5.9 & ~15.8 $\pm$ 5.9 & ~~~0.5  $\pm$  3.7 &   ~-6.8  $\pm$  4.0 &    ~~-0.3 $\pm$  3.6  &   ~-5.2 $\pm$  3.6  &   0.680 $\pm$  0.068  \\
\hline                                                                                                                                 
(53) CM-DRA             &  16 34 21.491 & +57 09 34.20 &                   &                  &-1109.0\tablenotemark{a} & 1203.0\tablenotemark{a} &               &                    &                      \\
(55) CM-DRA-REF45       &  16 33 57.769 & +57 14 22.96 &  ~~-9.4 $\pm$ 6.0 &  ~~6.1 $\pm$ 6.0 & ~-16.2  $\pm$  1.1 &   ~~9.2  $\pm$  2.4 &     ~-24.1 $\pm$  4.0  &   ~~2.5 $\pm$  4.0 &  2.648 $\pm$  0.265  \\
(26) CM-DRA-REF46       &  16 33 55.581 & +57 14 23.03 &  ~~~5.9 $\pm$ 6.0 &  ~~3.3 $\pm$ 6.0 & ~~-2.6  $\pm$  1.6 &   ~~2.4  $\pm$  1.9 &     ~~-9.1 $\pm$  4.0  &   ~-0.9 $\pm$  4.0 &                       \\
(54) CM-DRA-REF47       &  16 34 22.724 & +57 09 58.74 &                   &                  &-1109.0\tablenotemark{a} & 1203.0\tablenotemark{a} &  -1120.3 $\pm$ 4.1 & 1205.5 $\pm$ 4.1 & 60.976 $\pm$ 6.692  \\
(29) CM-DRA-REF58       &  16 33 44.428 & +57 12 46.05 &  ~~-6.9 $\pm$ 6.0 &  ~~4.7 $\pm$ 6.0 & ~-13.4  $\pm$  2.0 &  ~~1.1  $\pm$  2.2 &    ~-24.0 $\pm$ 14.1  &   -11.2 $\pm$ 14.1  &   1.365 $\pm$  0.136  \\
(30) CM-DRA-REF65       &  16 34 22.914 & +57 11 46.59 &  ~-13.9 $\pm$ 5.7 &  ~-9.0 $\pm$ 5.7 & ~-14.7  $\pm$  2.2 &   ~-6.6  $\pm$  2.5 &    ~-24.1 $\pm$  4.1  &   ~-7.4 $\pm$  4.1  &   1.279 $\pm$  0.128  \\
(31) CM-DRA-REF66       &  16 33 48.549 & +57 11 40.72 &  ~~~5.6 $\pm$ 6.0 &  ~22.5 $\pm$ 6.0 & ~~-2.4  $\pm$  1.0 &   ~14.1  $\pm$  1.4 &    ~~-8.6 $\pm$  4.0  &   ~17.4 $\pm$  4.0  &   1.432 $\pm$  0.144  \\
(32) CM-DRA-REF94       &  16 34 24.610 & +57 08 27.04 &  ~~~3.3 $\pm$ 5.7 &  ~-9.9 $\pm$ 5.7 & ~~-1.5  $\pm$  2.0 &   ~2.9  $\pm$  1.7 &     ~~-8.5 $\pm$  4.1  &   ~~4.4 $\pm$  4.1  &   0.149 $\pm$  0.019  \\
\hline                                                                                                                                 
(6)\phantom{4} TRES-HER0&  16 50 20.747 & +46 39 01.41 &  ~-28.6 $\pm$ 5.6  & ~28.2 $\pm$ 5.6  & ~-13.8  $\pm$  3.7 &   ~35.1  $\pm$  4.1 &    ~~-8.1 $\pm$  4.1  &   ~26.2 $\pm$  4.1  &                       \\
(44) TRES-HER0-REF337   &  16 50 03.825 & +46 43 17.03 &  ~~~1.8 $\pm$ 5.2  & ~~3.3 $\pm$ 5.2  & ~~~3.3  $\pm$  0.6 &   ~~4.5  $\pm$  1.5 &    ~~~2.3 $\pm$  1.3  &   ~~8.1 $\pm$  1.4  &   2.200 $\pm$  0.345  \\
(46) TRES-HER0-REF347   &  16 50 13.896 & +46 41 26.79 &  ~~-5.9 $\pm$ 5.3  & ~~7.4 $\pm$ 5.3  & ~~-7.6  $\pm$  3.9 &   ~~6.3  $\pm$  2.8 &    ~~~0.7 $\pm$  4.2  &   ~~4.3 $\pm$  4.2  &   1.249 $\pm$  0.125  \\
(52) TRES-HER0-REF363   &  16 50 58.822 & +46 38 49.05 &  ~-40.0 $\pm$ 5.3  & ~~2.7 $\pm$ 5.3  & ~-36.3  $\pm$  2.3 &   ~~5.1  $\pm$  6.9 &    ~-29.6 $\pm$  4.2  &   ~10.6 $\pm$  4.2  &   2.988 $\pm$  0.299  \\
(47) TRES-HER0-REF377   &  16 50 50.893 & +46 36 45.99 &  ~-41.3 $\pm$ 5.6  & ~36.4 $\pm$ 5.6  & ~-30.1  $\pm$  3.1 &   ~31.9  $\pm$  1.9 &    ~-25.9 $\pm$  4.1  &   ~31.4 $\pm$  4.1  &   2.754 $\pm$  0.275  \\
(48) TRES-HER0-REF380   &  16 50 48.223 & +46 36 31.92 &  ~-16.6 $\pm$ 5.6  & -11.9 $\pm$ 5.6  & ~~-5.3  $\pm$  2.9 &   -16.6  $\pm$  2.0 &    ~~-1.1 $\pm$  4.1  &   -16.4 $\pm$  4.1  &   0.435 $\pm$  0.043  \\
(49) TRES-HER0-REF394   &  16 49 56.224 & +46 33 36.01 &  ~~-1.8 $\pm$ 5.2  & -12.4 $\pm$ 5.2  & ~~~1.3  $\pm$  1.3 &   -15.1  $\pm$  0.9 &    ~~-2.4 $\pm$  1.6  &   -12.8 $\pm$  1.6  &   0.680 $\pm$  0.097  \\
(51) TRES-HER0-REF823   &  16 50 44.135 & +46 37 10.85 &  ~-20.9 $\pm$ 5.7  & -11.6 $\pm$ 5.7  & ~~-1.9  $\pm$ 14.5 &   ~-4.1  $\pm$ 16.1 &    ~~-6.0 $\pm$  4.1  &   -19.5 $\pm$  4.1  &   7.231 $\pm$  2.013  \\
\enddata 
\tablenotetext{a}{Proper motions from UCAC3}
\label{tab.initial}
\end{deluxetable*} 


==> tables/refstar_input_values.tex <==
%\LongTables % optionally

\begin{deluxetable*}{lrrrrrrrrrrrrrrr}
\rotate 
\tabletypesize{\tiny}
%\tabletypesize{\scriptsize}
\tablecaption{Initial star data used as constraints in the gaussfit astrometric model.}
\tablewidth{0pt}
\tablehead{
\colhead{Star} & \colhead{Gaia DR2}    & \colhead{$B-V$} & \colhead{$\sigma_{B-V}$} & \colhead{pmRA}     & \colhead{$\sigma_{\rm pmRA}$} & \colhead{pmDEC}    & \colhead{$\sigma_{\rm pmDEC}$} & \colhead{pmRA}     & \colhead{$\sigma_{\rm pmRA}$} & \colhead{pmDEC}    & \colhead{$\sigma_{\rm pmDEC}$} & \colhead{$\pi$}    & \colhead{$\sigma_\pi$} & \colhead{$\pi$} & \colhead{$\sigma_\pi$} \\
\colhead{}     & \colhead{Designation} & \colhead{(mag)} & \colhead{(mag)}         & \colhead{UCAC5}    & \colhead{UCAC5}            & \colhead{UCAC5}    & \colhead{UCAC5}             & \colhead{Gaia DR2} & \colhead{Gaia DR2}          & \colhead{Gaia DR2} & \colhead{Gaia DR2}          & \colhead{Gaia DR2} & \colhead{Gaia}        & \colhead{SpecPhot} & \colhead{SpecPhot}\\
\colhead{}     & \colhead{}            & \colhead{}      & \colhead{}              & \colhead{(mas/yr)} & \colhead{(mas/yr)}         & \colhead{(mas/yr)} & \colhead{(mas/yr)}          & \colhead{(mas/yr)} & \colhead{(mas/yr)}          & \colhead{(mas/yr)} & \colhead{(mas/yr)}          & \colhead{(mas)}      & \colhead{(mas)}     & \colhead{(mas)}      & \colhead{(mas)}    }               
\startdata
(2)  YY-GEM            &   892348454394856064  &  1.454 &  0.010  &    -204.5  &  3.1 &  -100.9 &  3.1 &  -201.490 &  0.087 &   -97.104 &  0.074  &   66.2323 &  0.0511 &  71.40 & 14.28  \\
(7)  YY-GEM-REF1       &   892301823941440384  &  1.095 &  0.023  &       1.5  &  1.0 &    -1.8 &  1.0 &     2.167 &  0.068 &    -2.568 &  0.061  &    0.8831 &  0.0395 &   0.86 &  0.17  \\ 
(8)  YY-GEM-REF2       &   892301793870145920  &  0.651 &  0.026  &       1.0  &  1.0 &    -3.8 &  1.0 &     1.423 &  0.059 &    -3.827 &  0.053  &    2.4443 &  0.0357 &   2.13 &  0.43  \\ 
(9)  YY-GEM-REF3       &   892347045645587456  &  0.932 &  0.047  &      -1.2  &  1.2 &    -6.0 &  1.2 &    -2.489 &  0.072 &    -4.239 &  0.063  &    1.0794 &  0.0438 &   1.26 &  0.25  \\ 
(10) YY-GEM-REF4       &   892348312664063616  &  0.804 &  0.093  &       0.4  &  1.3 &    -3.9 &  1.3 &     0.168 &  0.055 &    -3.866 &  0.055  &    0.7035 &  0.0316 &   1.02 &  0.20  \\ 
(11) YY-GEM-REF5       &   892348420035116416  &  0.307 &  0.999  &       1.9  &  5.5 &   -15.0 &  5.4 &     0.865 &  0.138 &    -8.020 &  0.123  &    0.8158 &  0.0842 &   0.42 &  0.08  \\ 
(12) YY-GEM-REF6       &   892348415740921344  &  0.569 &  0.679  &       0.6  &  4.1 &   -12.4 &  4.2 &           &        &           &         &           &         &   0.56 &  0.11  \\ 
(13) YY-GEM-REF7       &   892348553182232320  &  1.066 &  0.468  &      -9.2  &  2.4 &   -28.7 &  2.4 &    -6.523 &  0.048 &   -26.047 &  0.038  &    2.0399 &  0.0312 &   2.23 &  0.45  \\ 
(5)\phantom{3} NSVS0103&  1715299716278321408  &  1.541 &  0.244  &    -108.1  &  1.6 &    58.7 &  1.6 &  -106.773 &  0.063 &    58.861 &  0.051  &   16.4797 &  0.0304 &   7.10 &  1.42  \\
(33) NSVS0103-REF00    &  1715294768475996160  &  0.771 &  0.018  &       8.3  &  1.7 &     6.3 &  1.7 &     6.445 &  0.033 &     7.304 &  0.025  &    2.0480 &  0.0152 &   2.10 &  0.42  \\
(34) NSVS0103-REF01    &  1715287690369845248  &  0.698 &  0.019  &       8.5  &  1.9 &   -14.0 &  1.9 &     5.741 &  0.035 &   -17.192 &  0.026  &    1.3864 &  0.0163 &   1.49 &  0.30  \\
(35) NSVS0103-REF02    &  1715287445555837568  &  0.691 &  0.015  &     -40.0  &  1.5 &     9.5 &  1.5 &   -38.722 &  0.062 &    10.452 &  0.052  &    6.7977 &  0.0299 &   7.58 &  1.52  \\
(36) NSVS0103-REF05    &  1715281986653319936  &  0.917 &  0.024  &      -9.2  &  2.2 &    -2.6 &  2.2 &    -7.519 &  0.039 &    -4.500 &  0.031  &    2.2603 &  0.0182 &   2.08 &  0.42  \\
(37) NSVS0103-REF19    &  1715280955861122304  &  0.709 &  0.019  &      -2.0  &  1.7 &     2.6 &  1.7 &    -3.117 &  0.034 &     0.993 &  0.024  &    0.8307 &  0.0135 &   1.94 &  0.39  \\
(41) NSVS0103-REF23    &  1715281436897503744  &  0.573 &  0.014  &       4.3  &  1.5 &    -1.3 &  1.5 &     4.315 &  0.046 &    -1.027 &  0.037  &    1.7803 &  0.0218 &   2.26 &  0.45  \\
(39) NSVS0103-REF68    &  1715287999607537408  &  1.522 &  0.045  &    -116.1  &  4.0 &    59.0 &  3.5 &  -107.709 &  0.099 &    59.721 &  0.080  &   16.5720 &  0.0476 &  18.87 &  3.77  \\
(40) NSVS0103-REF96    &  1715287003175078528  &  0.504 &  0.020  &      -5.8  &  1.6 &     5.5 &  1.6 &    -6.897 &  0.049 &     4.469 &  0.041  &    0.8758 &  0.0263 &   1.34 &  0.27  \\
(1)\phantom{2}  GU-BOO &  1278589709364139520  &  1.252 &  0.028  &      23.7  &  1.3 &   -29.4 &  1.2 &    22.728 &  0.022 &   -30.809 &  0.031  &    6.1468 &  0.0159 &   7.10 &  1.42  \\
(20) GU-BOO-REF01      &  1278596821829967232  &  0.913 &  0.026  &      -0.3  &  3.9 &     5.2 &  3.0 &    -1.748 &  0.317 &     1.243 &  0.438  &    1.9713 &  0.2398 &   2.08 &  0.42  \\
(21) GU-BOO-REF05      &  1278590946314709376  &  0.947 &  0.049  &     -14.6  &  2.4 &    18.3 &  2.5 &   -15.284 &  0.032 &    11.051 &  0.049  &    1.4348 &  0.0263 &   1.46 &  0.29  \\
(22) GU-BOO-REF08      &  1278595997196243968  &  0.592 &  0.032  &     -99.9  &  1.3 &     5.5 &  1.3 &   -98.846 &  0.051 &     4.760 &  0.085  &    2.4030 &  0.0406 &   1.45 &  0.29  \\
(19) GU-BOO-REF25      &  1278596031555984512  &  1.020 &  0.030  &      -5.3  &  2.0 &     0.5 &  2.0 &    -3.183 &  0.029 &    -0.532 &  0.045  &    1.7436 &  0.0226 &   2.27 &  0.45  \\
(18) GU-BOO-REF51      &  1278585448756580992  &  1.035 &  0.031  &     -12.4  &  1.3 &    18.1 &  1.4 &   -11.744 &  0.030 &    16.725 &  0.041  &    5.1188 &  0.0218 &   5.05 &  1.01  \\
(15) GU-BOO-REF53      &  1278590121680984576  &  0.569 &  0.031  &       5.2  &  1.8 &   -13.7 &  1.8 &     4.186 &  0.026 &   -16.624 &  0.040  &    1.0645 &  0.0197 &   0.92 &  0.18  \\
(14) GU-BOO-REF57      &  1278589640644642432  &  0.633 &  0.031  &      -3.1  &  2.3 &     2.3 &  2.3 &    -4.410 &  0.034 &    -1.289 &  0.050  &    0.6850 &  0.0250 &   0.74 &  0.15  \\
(53) CM-DRA            &  1431176943768690816  &  1.532 &  0.007  &   -1109.0  & 11.0 &  1203.0 & 12.0 & -1113.612 &  0.114 &  1181.211 &  0.100  &   67.3400 &  0.0514 &  62.50 & 12.50  \\
(55) CM-DRA-REF45      &  1431189656871892992  &  0.821 &  0.011  &     -14.4  &  1.4 &    -0.4 &  1.5 &   -16.144 &  0.034 &     0.948 &  0.027  &    0.5904 &  0.0158 &   3.89 &  0.78  \\
(26) CM-DRA-REF46      &  1431189725591369600  &  0.618 &  0.014  &      -6.7  &  1.8 &    -5.4 &  1.7 &    -0.988 &  0.436 &    -5.548 &  0.375  &    1.9460 &  0.2039 &   1.15 &  0.23  \\
(54) CM-DRA-REF47      &  1431176943768691328  &  0.472 &  0.028  &   -1109.0  & 11.0 &  1203.0 & 12.0 & -1110.868 &  0.048 &  1199.405 &  0.043  &   67.3216 &  0.0233 &  60.98 & 13.38  \\
(29) CM-DRA-REF58      &  1431189519432936064  &  0.700 &  0.022  &     -17.0  &  1.9 &    -5.4 &  2.0 &   -14.963 &  0.051 &    -2.446 &  0.038  &    1.2031 &  0.0226 &   1.39 &  0.28  \\
(30) CM-DRA-REF65      &  1431188797878430720  &  0.850 &  0.023  &     -11.1  &  3.2 &   -13.1 &  3.7 &   -14.704 &  0.060 &    -9.449 &  0.049  &    1.3518 &  0.0322 &   1.36 &  0.27  \\
(31) CM-DRA-REF66      &  1431189313274504576  &  0.556 &  0.011  &       0.0  &  1.5 &    12.0 &  1.5 &    -0.800 &  0.057 &    14.745 &  0.050  &    1.0338 &  0.0289 &   1.72 &  0.34  \\
(32) CM-DRA-REF94      &  1431176600171304448  &  0.960 &  0.015  &       0.6  &  1.7 &    -1.4 &  1.7 &    -0.744 &  0.036 &    -1.938 &  0.033  &    0.1699 &  0.0181 &   0.18 &  0.04  \\
(6)\phantom{4} TRES-HER0& 1407718450873494784  &  1.477 &  0.056  &     -15.1  &  3.1 &    26.6 &  3.1 &   -12.075 &  0.070 &    29.904 &  0.088  &    7.1126 &  0.0382 &   8.50 &  1.70  \\
(44) TRES-HER0-REF337  &  1407722642761588608  &  0.467 &  0.012  &       4.2  &  1.3 &     4.2 &  1.3 &     4.082 &  0.048 &     3.242 &  0.055  &    1.8626 &  0.0267 &   2.58 &  0.52  \\
(46) TRES-HER0-REF347  &  1407719516025390208  &  0.602 &  0.011  &      -2.0  &  1.5 &     5.8 &  1.5 &    -3.679 &  0.030 &     5.232 &  0.036  &    0.7611 &  0.0162 &   1.42 &  0.28  \\
(52) TRES-HER0-REF363  &  1407708074232494976  &  0.949 &  0.013  &     -31.2  &  1.5 &     7.3 &  1.5 &   -32.537 &  0.040 &     6.398 &  0.058  &    3.0533 &  0.0225 &   3.04 &  0.61  \\
(47) TRES-HER0-REF377  &  1407705806489762432  &  0.874 &  0.013  &     -28.1  &  1.4 &    33.8 &  1.4 &   -27.801 &  0.027 &    32.730 &  0.041  &    2.5503 &  0.0164 &   3.04 &  0.61  \\
(48) TRES-HER0-REF380  &  1407705806489762944  &  0.557 &  0.009  &      -2.8  &  1.5 &   -15.3 &  1.5 &    -4.005 &  0.035 &   -16.794 &  0.050  &    0.8594 &  0.0205 &   0.25 &  0.05  \\
(49) TRES-HER0-REF394  &  1407711991242771200  &  0.733 &  0.046  &       2.8  &  1.3 &   -14.8 &  1.3 &     2.228 &  0.041 &   -14.657 &  0.052  &    0.8895 &  0.0223 &   0.73 &  0.15  \\
(51) TRES-HER0-REF823  &  1407706592467909632  &  1.088 &  0.012  &      -3.2  &  2.4 &   -19.7 &  2.4 &    -6.813 &  0.054 &   -16.318 &  0.077  &    0.1902 &  0.0316 &   0.84 &  0.17  \\
\enddata                                                                                
\label{tab.input}

\tablecomments{XXX We need explanations here plus a reference to the relevant section(s) of the paper.}

\end{deluxetable*} 


==> tables/refstar_spt_phot.tex <==
\begin{deluxetable*}{llllll}
%\tabletypesize{\tiny}
%\tabletypesize{\scriptsize}
\tablecaption{Spectral types and $BVRI$ photometry of the astrometric reference stars}
\tablewidth{0pt}
\tablehead{
\colhead{Star}          & \colhead{SpT} & \colhead{$B$}      & \colhead{$V$}      & \colhead{$R$}      & \colhead{$I$}        \\
\colhead{}              & \colhead{}    & \colhead{(mag)}    & \colhead{(mag)}    & \colhead{(mag)}    & \colhead{(mag)}   }
\startdata
%(2)  YY-GEM            &   M1.0Ve    &  \nodata             & \nodata            & \nodata            & \nodata              \\             
(7)  YY-GEM-REF1        &   K0IIIb    &  12.265 $\pm$ 0.018             & 11.170 $\pm$ 0.014            & 10.617 $\pm$ 0.044            & 10.045 $\pm$ 0.044              \\
(8)  YY-GEM-REF2        &   G3V       &  13.557 $\pm$ 0.022             & 12.906 $\pm$ 0.013            & 12.616 $\pm$ 0.021            & 12.218 $\pm$ 0.021              \\
(9)  YY-GEM-REF3        &   K0III     &  10.860 $\pm$ 0.019             & 9.928 $\pm$ 0.043             & 9.448 $\pm$ 0.041            & 8.893 $\pm$ 0.007              \\
(10) YY-GEM-REF4        &   G0V       &  14.699 $\pm$ 0.006             & 13.895 $\pm$ 0.093            & 13.586 $\pm$ 0.182            & 13.343 $\pm$ 0.182              \\
(11) YY-GEM-REF5        &   G0V?      &  16.658 $\pm$ 0.636             & 16.351 $\pm$ 0.770            & 15.927 $\pm$ 0.644            & 15.559 $\pm$ 0.433              \\
(12) YY-GEM-REF6        &   G2V       &  15.410 $\pm$ 0.442             & 14.841 $\pm$ 0.515            & 14.859 $\pm$ 0.495            & 13.956 $\pm$ 0.278              \\
(13) YY-GEM-REF7        &   G8V       &  14.761 $\pm$ 0.340             & 13.695 $\pm$ 0.322            & 13.482 $\pm$ 0.302            & 12.984 $\pm$ 0.185              \\
\hline                                                                                                      
%(5)\phantom{3} NSVS0103 &  M2-M3V    &   15.063 $\pm$ 0.225 & 13.522 $\pm$ 0.094 & 12.461 $\pm$ 0.198 & 11.158 $\pm$ 0.271  \\
(33) NSVS0103-REF00     &   G8V       &   14.535 $\pm$ 0.014 & 13.764 $\pm$ 0.011 & 13.313 $\pm$ 0.015 & 12.947 $\pm$ 0.044  \\
(34) NSVS0103-REF01     &   G5V       &   15.001 $\pm$ 0.015 & 14.303 $\pm$ 0.012 & 13.889 $\pm$ 0.017 & 13.528 $\pm$ 0.040  \\
(35) NSVS0103-REF02     &   G5V       &   11.465 $\pm$ 0.013 & 10.774 $\pm$ 0.007 & 10.375 $\pm$ 0.016 & 10.017 $\pm$ 0.031  \\
(36) NSVS0103-REF05     &   K2V       &   15.697 $\pm$ 0.022 & 14.780 $\pm$ 0.009 & 14.218 $\pm$ 0.020 & 13.743 $\pm$ 0.062  \\
(37) NSVS0103-REF19     &   G3V       &   14.367 $\pm$ 0.015 & 13.658 $\pm$ 0.012 & 13.227 $\pm$ 0.020 & 12.849 $\pm$ 0.040  \\
(41) NSVS0103-REF23     &   G0V       &   13.195 $\pm$ 0.011 & 12.622 $\pm$ 0.009 & 12.277 $\pm$ 0.016 & 11.967 $\pm$ 0.029  \\
(39) NSVS0103-REF68     &   M4.5V     &   17.300 $\pm$ 0.042 & 15.778 $\pm$ 0.015 & 14.528 $\pm$ 0.030 & 13.006 $\pm$ 0.021  \\
(40) NSVS0103-REF96     &   F6V       &   13.522 $\pm$ 0.015 & 13.018 $\pm$ 0.013 & 12.706 $\pm$ 0.016 & 12.429 $\pm$ 0.038  \\
\hline                                                                                                                     
%(1)\phantom{2} GU-BOO  &   M0/M1.5V  &   14.903 $\pm$ 0.019 & 13.651 $\pm$ 0.020 & 12.918 $\pm$ 0.108 & 12.089 $\pm$ 0.071  \\
(20) GU-BOO-REF01       &   K0V       &   15.563 $\pm$ 0.019 & 14.650 $\pm$ 0.018 & 14.104 $\pm$ 0.011 & 13.629 $\pm$ 0.022  \\
(21) GU-BOO-REF05       &   K0-K2V    &   16.348 $\pm$ 0.046 & 15.401 $\pm$ 0.016 & 14.861 $\pm$ 0.022 & 14.366 $\pm$ 0.071  \\
(22) GU-BOO-REF08       &   F9V       &   14.438 $\pm$ 0.026 & 13.846 $\pm$ 0.019 & 13.446 $\pm$ 0.011 & 13.027 $\pm$ 0.011  \\
(19) GU-BOO-REF25       &   K3V       &   16.278 $\pm$ 0.025 & 15.258 $\pm$ 0.017 & 14.620 $\pm$ 0.020 & 14.132 $\pm$ 0.008  \\
(18) GU-BOO-REF51       &   K3V       &   14.286 $\pm$ 0.024 & 13.251 $\pm$ 0.020 & 12.640 $\pm$ 0.017 & 12.130 $\pm$ 0.005  \\
(15) GU-BOO-REF53       &   G0V       &   15.241 $\pm$ 0.025 & 14.672 $\pm$ 0.018 & 14.324 $\pm$ 0.016 & 13.995 $\pm$ 0.020  \\
(14) GU-BOO-REF57       &   G2V       &   15.952 $\pm$ 0.028 & 15.319 $\pm$ 0.014 & 14.960 $\pm$ 0.014 & 14.643 $\pm$ 0.089  \\
\hline                                                                                                                     
%(53) CM-DRA            &   M4.5V     &   14.448 $\pm$ 0.007 & 12.916 $\pm$ 0.002 & 11.626 $\pm$ 0.006 &  9.987 $\pm$ 0.039  \\
(55) CM-DRA-REF45       &   G8V?      &   14.231 $\pm$ 0.006 & 13.410 $\pm$ 0.009 & 12.935 $\pm$ 0.010 & 12.467 $\pm$ 0.004  \\
(26) CM-DRA-REF46       &   G2V       &   14.929 $\pm$ 0.004 & 14.311 $\pm$ 0.013 & 13.950 $\pm$ 0.008 & 13.617 $\pm$ 0.004  \\
(54) CM-DRA-REF47       &   WD        &   15.501 $\pm$ 0.020 & 15.029 $\pm$ 0.020 & 14.710 $\pm$ 0.007 & 14.394 $\pm$ 0.061  \\
(29) CM-DRA-REF58       &   G5-G6V    &   15.283 $\pm$ 0.015 & 14.583 $\pm$ 0.016 & 14.186 $\pm$ 0.009 & 13.810 $\pm$ 0.040  \\
(30) CM-DRA-REF65       &   K0V       &   16.167 $\pm$ 0.022 & 15.317 $\pm$ 0.008 & 14.842 $\pm$ 0.006 & 14.416 $\pm$ 0.052  \\
(31) CM-DRA-REF66       &   F9V       &   13.464 $\pm$ 0.007 & 12.908 $\pm$ 0.009 & 12.585 $\pm$ 0.009 & 12.264 $\pm$ 0.008  \\
(32) CM-DRA-REF94       &   K0III     &   15.332 $\pm$ 0.012 & 14.372 $\pm$ 0.009 & 13.836 $\pm$ 0.005 & 13.356 $\pm$ 0.006  \\
\hline                                                                                                                     
%(6)\phantom{4} TRES-HER0&  M2-M3 V   &   17.233 $\pm$ 0.050 & 15.756 $\pm$ 0.025 & 14.578 $\pm$ 0.022 & 13.135 $\pm$ 0.041  \\
(44) TRES-HER0-REF337   &   F5V       &   11.861 $\pm$ 0.003 & 11.394 $\pm$ 0.012 & 11.108 $\pm$ 0.015 & 10.825 $\pm$ 0.002  \\
(46) TRES-HER0-REF347   &   G0V       &   14.478 $\pm$ 0.008 & 13.876 $\pm$ 0.008 & 13.507 $\pm$ 0.015 & 13.152 $\pm$ 0.008  \\
(52) TRES-HER0-REF363   &   K3V       &   15.169 $\pm$ 0.005 & 14.220 $\pm$ 0.012 & 13.632 $\pm$ 0.017 & 13.126 $\pm$ 0.005  \\
(47) TRES-HER0-REF377   &   K0V       &   14.428 $\pm$ 0.008 & 13.554 $\pm$ 0.010 & 13.075 $\pm$ 0.014 & 12.661 $\pm$ 0.003  \\
(48) TRES-HER0-REF380   &   F8III     &   14.674 $\pm$ 0.006 & 14.117 $\pm$ 0.007 & 13.784 $\pm$ 0.014 & 13.457 $\pm$ 0.006  \\
(49) TRES-HER0-REF394   &   K2IIIab   &   12.013 $\pm$ 0.004 & 10.925 $\pm$ 0.011 & 10.361 $\pm$ 0.019 &  9.849 $\pm$ 0.010  \\
(51) TRES-HER0-REF823   &   G2V       &   16.196 $\pm$ 0.028 & 15.463 $\pm$ 0.037 & 15.010 $\pm$ 0.028 & 14.602 $\pm$ 0.046  \\
\enddata 
\label{tab.phot}
\end{deluxetable*} 


==> tables/target_information.tex <==
%% LaTeX deluxetable generator for the AASTeX package.
%% Written by Greg Schwarz (5/1/2001).

%% Table generated: Mon Sep  6 22:47:06 2010

%% Remove the two lines and the last line if you want
%% want to incorporate this table into another LaTex document.
%\documentclass[twocolumn]{emulateapj}
%\begin{document}

%% The values (usually only l,r and c) in the last part of
%% \begin{deluxetable}{} command tell LaTeX how many columns
%% there are and how to align them.
\begin{deluxetable*}{lllccccccl}

%% Keep a portrait orientation

%% Over-ride the default font size
%% Use Default (12pt)

%% Use \tablewidth{?pt} to over-ride the default table width.
%% If you are unhappy with the default look at the end of the
%% *.log file to see what the default was set at before adjusting
%% this value.

%% This is the title of the table.
\tablecaption{\label{tab_targetStarsInfo}Observed targets, coordinates, $V$-band magnitude, primary and secondary masses, orbital period and separation, and distance as given in cited reference.}

%% This command over-rides LaTeX's natural table count
%% and replaces it with this number.  LaTeX will increment
%% all other tables after this table based on this number
%% \tablenum{1}

%% The \tablehead gives provides the column headers.  It
%% is currently set up so that the column labels are on the
%% top line and the units surrounded by ()s are in the
%% bottom line.  You may add more header information by writing
%% another line between these lines. For each column that requries
%% extra information be sure to include a \colhead{text} command
%% and remember to end any extra lines with \\ and include the
%% correct number of &s.
\tablehead{\colhead{Target} & \colhead{RA} & \colhead{DE} & \colhead{V} & \colhead{$M_1$} & \colhead{$M_2$} & \colhead{$P$} & \colhead{$a$} & \colhead{$\pi$} & \colhead{Reference} \\
\colhead{} & \colhead{(hms)} & \colhead{(dms)} & \colhead{(mag)} & \colhead{($M_\odot$)} & \colhead{($M_\odot$)} & \colhead{(days)} & \colhead{(AU)} & \colhead{(mas)} & \colhead{} }

%% All data must appear between the \startdata and \enddata commands
\startdata
YY Gem     &  07 34 37.41  &   +31 52 09.79   &  10.7  &  0.599  &  0.599  &  0.8143  &  0.0181  &  71.4  &    Torres \& Ribas 2002  \\
NSVS0103   &  13 45 34.89  &   +79 23 48.28  &  13.4  &  0.543  &  0.498  &  0.3681  &  0.0102  &  7.1  &    Lopez-Morales et al (2006)  \\
GU Boo     &  15 21 55.17  &   +33 56 04.20   &  13.6  &  0.610  &  0.599  &  0.4887  &  0.0129  &  7.1  &    Lopez-Morales \& Ribas (2005)  \\
CM Dra     &  16 34 20.35  &   +57 09 44.70  &  12.9  &  0.231  &  0.214  &  1.2684  &  0.0175  &  62.5  &    Metcalfe et al (1996)  \\
TrES-Her0  &  16 50 20.75  &   +46 39 01.39   &  15.5  &  0.493  &  0.489  &  1.12079  &  0.0105  &  8.5  &    Creevey et al (2005)  \\
\enddata

%% Include any \tablenotetext{key}{text}, \tablerefs{ref list},
%% or \tablecomments{text} between the \enddata and
%% \end{deluxetable} commands

%% No \tablecomments indicated

%% No \tablerefs indicated

\end{deluxetable*}
%\end{document}

